Don't Push the Button! Exploring Data Leakage Risks in Machine Learning and Transfer Learning

Machine Learning (ML) has revolutionized various domains, offering predictive capabilities in several areas. However, with the increasing accessibility of ML tools, many practitioners, lacking deep ML expertise, adopt a "push the button" approach, utilizing user-friendly interfaces without a thorough understanding of underlying algorithms. While this approach provides convenience, it raises concerns about the reliability of outcomes, leading to challenges such as incorrect performance evaluation. This paper addresses a critical issue in ML, known as data leakage, where unintended information contaminates the training data, impacting model performance evaluation. Users, due to a lack of understanding, may inadvertently overlook crucial steps, leading to optimistic performance estimates that may not hold in real-world scenarios. The discrepancy between evaluated and actual performance on new data is a significant concern. In particular, this paper categorizes data leakage in ML, discussing how certain conditions can propagate through the ML workflow. Furthermore, it explores the connection between data leakage and the specific task being addressed, investigates its occurrence in Transfer Learning, and compares standard inductive ML with transductive ML frameworks. The conclusion summarizes key findings, emphasizing the importance of addressing data leakage for robust and reliable ML applications.

==> TAB_SUMMARY_TREE1.tex <==
\begin{forest}
  for tree={
    font=\scriptsize,
    grow=east,
    edge path={
      \noexpand\path [draw, \forestoption{edge}] (!u.east) -- ++(2pt,0) |- (.west)\forestoption{edge label};
    },
    parent anchor=east,
    child anchor=west,
    l sep=15pt,
    s sep=10pt,
    anchor=west,
    tier/.pgfmath=level(),
    rectangle,
    rounded corners,
    draw,
    fill=white,
    text width=13.3em,
    minimum height=5em,
    align=left,
    inner sep=4pt,
  }
  [\textbf{Data-induced leakage}\\
  Spurious information embedded\\ in the data already\\ during the dataset construction. \\
    [\textbf{Data collecting leakage}\\
    The process of data collecting\\ introduces spurious information\\ or unintended dependencies \\influencing the model learning.\\
    ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{roberts2021common,li2020perils}}}]
    [\textbf{Synthesis leakage}\\
    The ML pipeline involves\\ the generation of new data\\ in training and evaluation sets\\ accessing to knowledge from \\the same data instances.
    ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{yang2022data,bouke2023empirical}}}
      %[\textbf{Oversample leakage}\\
      %Data instances used to evaluate \\ the final model are also exploited\\ by the oversampling method.\\
      %,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{yang2022data,bouke2023empirical}}}]
      %[\textbf{Undersample leakage}\\
      %Removal of data instances made \\ relying on out-of-training data.\\
      %,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{yang2022data}}}]
    ]
    [\textbf{Label leakage}\\
    The real label is embedded\\ within the chosen data\\  representation.\\
    ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{kapoor2023leakage}}}
      [\textbf{Direct label leakage}\\
      Data representations contain\\ features corresponding to\\ the real label.\\
      ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{rosset2010medical}}}]
      [\textbf{Indirect label leakage}\\
      There exist features in data\\ instances s.t. are spurious or \\encoding information derived\\ from the real label.\\
      ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{chiavegatto2021data}}}]
    ]
  ]
\end{forest}

==> TAB_SUMMARY_TREE2.tex <==
\begin{forest}
  for tree={
    font=\scriptsize,
    grow=east,
    edge path={
      \noexpand\path [draw, \forestoption{edge}] (!u.east) -- ++(2pt,0) |- (.west)\forestoption{edge label};
    },
    parent anchor=east,
    child anchor=west,
    l sep=15pt,
    s sep=10pt,
    anchor=west,
    tier/.pgfmath=level(),
    rectangle,
    rounded corners,
    draw,
    fill=white,
    text width=16em,
    minimum height=1em,
    align=left,
    inner sep=6pt,
  }
  [\textbf{Preprocessing-related leakage}\\
  A pre-processing function operates on \\ the dataset using information derived \\ from the whole input dataset.\\
    [\textbf{Normalization leakage}\\
    A normalization function is applied\\ to each data point using parameters \\ calculated over the entire dataset.\\
    ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{yang2022data}}}]
    [\textbf{Cleaning leakage}\\
    A cleaning function is applied to each \\ data point using parameters calculated\\ over the entire dataset.\\,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{kuhn2019feature}}}]
    [\textbf{Imputation leakage}\\
    An imputation function is applied to \\ each data point using parameters \\ calculated over the entire dataset.\\
    ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{kapoor2023leakage}}}]
    [\textbf{Feature engineering leakage}\\
    A feature engineering strategy relies \\ also on data used in the evaluation step.\\
    ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{shim2021inflated}}}]
  ]
\end{forest}

==> TAB_SUMMARY_TREE3.tex <==

\begin{forest}
  for tree={
    font=\scriptsize,
    grow=east,
    edge path={
      \noexpand\path [draw, \forestoption{edge}] (!u.east) -- ++(2pt,0) |- (.west)\forestoption{edge label};
    },
    parent anchor=east,
    child anchor=west,
    l sep=15pt,
    s sep=10pt,
    anchor=west,
    tier/.pgfmath=level(),
    rectangle,
    rounded corners,
    draw,
    fill=white,
    text width=14em,
    minimum height=1em,
    align=left,
    inner sep=6pt,
  }
  [\textbf{Split-related leakage}\\
  Leak of information between\\ training and evaluation sets \\ can occur during\\ the split procedure.\\
    [\textbf{Distribution leakage}\\
    The data split reduces\\ data distribution differences\\ making them unrepresentative\\of the real-world task.\\
    ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.55cm,yshift=-0.9cm,yshift=10pt]{\cite{kapoor2023leakage,plotz2021applying,lyu2021empirical}}}]
    [\textbf{Similarity leakage}\\
    Similarities or connections between \\ data instances in different sets\\ are present.\\
    ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{lee2018validity,plotz2021applying}}}
      [\textbf{Sets' intersection leakage}\\
      Training and out-of-the-training \\ data contain a part or all of the \\ same data instances.\\
      ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{lee2018validity}}}]
      [\textbf{Overlap leakage}\\
      instances in the out-of-the-training \\sets are partially composed\\ of segments or features originating\\ from instances in the training set.\\
      ,edge label={node[midway,above,rotate=90,font=\tiny,xshift=0.35cm,yshift=-0.9cm,yshift=10pt]{\cite{plotz2021applying}}}]
    ]
  ]
\end{forest}
